Are We Paying Attention to Her? Investigating Gender Disambiguation and Attention in Machine Translation

While gender bias in modern Neural Machine Translation (NMT) systems has received much attention, traditional evaluation metrics do not to fully capture the extent to which these systems integrate contextual gender cues. We propose a novel evaluation metric called Minimal Pair Accuracy (MPA), which measures the reliance of models on gender cues for gender disambiguation. MPA is designed to go beyond surface-level gender accuracy metrics by focusing on whether models adapt to gender cues in minimal pairs -- sentence pairs that differ solely in the gendered pronoun, namely the explicit indicator of the target's entity gender in the source language (EN). We evaluate a number of NMT models on the English-Italian (EN--IT) language pair using this metric, we show that they ignore available gender cues in most cases in favor of (statistical) stereotypical gender interpretation. We further show that in anti-stereotypical cases, these models tend to more consistently take masculine gender cues into account while ignoring the feminine cues. Furthermore, we analyze the attention head weights in the encoder component and show that while all models encode gender information to some extent, masculine cues elicit a more diffused response compared to the more concentrated and specialized responses to feminine gender cues.

==> notes/old_related_work.tex <==
%Overview of prior work on:
%- Gender bias in machine translation and gender disambiguation\\
%- \ev{I think it makes sense to write such a section since you can use if for your PhD anyways but you might not need this in this particular paper (especially not if it's a short paper). You can focus on specific work related to interpretability maybe!}
%\chiara{I agree, I tried to include some information in the Introduction to explain the broader context, I will keep the related work section focused on Interpretability (an specifically in MT).}

%- Interpretability methods (e.g., from probing to attribution methods, attention, value zeroing..., specifically to MT...)\\

Gender bias has been extensively documented across NLP tasks, including Machine Translation \citep{bias1, bias3, bias4, winomt, bias6}. Over the past decade, various bias mitigation strategies have been proposed \citep{cda,bias2,costa_jussa, bias6, basta, reinflection, lattice, parataxis}, predominantly operating at the pre- or post-processing stage - either by artificially manipulating training data or by correcting translations once generated. However, these methods have shown limited success - often addressing specific issues without generalizing effectively - and their relevance is frequently questioned, particularly when biases observed in downstream tasks do not clearly correlate with the interventions applied \citep{biased_rulers}.

Attempts to control gender bias by intervening directly in model internals remain rare. For instance, \citet{bau} sought to manipulate gender in MT by probing and deactivating specific neurons correlated with gender information. However, gender properties were found to be highly distributed across the network, thus complicating targeted control. Notably, the study was based on LSTM architectures rather than Transformer models that now dominate modern MT and general-purpose LLMs. More recently, \citet{van-der-wal-etal-2022-birth} explored the evolution of gender representation and the resulting bias within the same architecture. Although their findings do not directly pertain to MT, they observe an asymmetry in how gender information is encoded, with feminine entities appearing to be represented more locally.

In this context, interpretability techniques may help understanding model decisions, diagnosing biases, and informing debiasing strategies. Specifically to MT, research has focused on linguistic competence through probing \citep{belinkov-etal-2017-neural,belinkov-etal-2017-evaluating, conneau-etal-2018-cram}, or by analyzing contrastive translation \citep{sennrich-2017-grammatical, vamvas-sennrich-2021-contrastive, vamvas-sennrich-2022-little, burlot-yvon-2017-evaluating, rios-gonzales-etal-2017-improving}. More recent work has investigated how MT systems process intra- and inter-sentential context and whether their context usage aligns with human expectations \citep{goindani-shrivastava-2021-dynamic, voita-etal-2021-analyzing, sarti2024_context, mohammed-niculae-2024-measuring}. Despite high overall performance, these studies highlight how models often struggle to effectively leverage contextual information, either failing to integrate necessary information or attending to irrelevant tokens when resolving ambiguities \citep{kim-etal-2019-document, yin-etal-2021-context}. This raises concerns about whether gender disambiguation in MT is truly driven by meaningful context usage or biased statistical patterns. 

The problem of context integration is not only relevant to model decision-making but also affects how gender bias is evaluated. Template-based evaluation frameworks, such as WinoMT \citep{winomt}, provide controlled settings to measure surface-level accuracy metrics, and have been widely used to quantify gender bias across different language pairs and MT systems \citep{kocmi-etal-2020-gender, costajussa2020, choubey-etal-2021-gfst}. However, as these primarily rely on the alignment and morphosyntactic analysis of ambiguous words, they do not reveal whether models actively integrate contextual cues when making gender-related decisions. These limitations underscore the need for more nuanced evaluation methods.

A promising avenue for investigating how gender cues influence model decisions is through the study of context mixing, i.e., the ability of Transformer-based models to dynamically incorporate information from the broader context into token representations. This process is largely governed by the attention mechanism, which plays a central role in these models. While attention-based analyses  have been criticized for their reliability \citep{jain-wallace-2019-attention, bibal-etal-2022-attention}, and more advanced interpretability methods have been introduced \citep{kobayashi-etal-2020-attention, kobayashi-etal-2021-incorporating, modarressi-etal-2022-globenc, ferrando-etal-2022-measuring, mohebbi-etal-2023-quantifying}, self-attention weights remain a popular choice for analyzing model behavior due to their ability to provide direct insights into token interactions across layers and heads. As a matter of fact, they have been extensively leveraged to track token dependencies, revealing that specific attention heads may specialize in distinct linguistic functions \citep{clark-etal-2019-bert, kovaleva-etal-2019-revealing, reif2019, lin-etal-2019-open, attention2017, voita-etal-2019-analyzing, xu2015, wang2016, lee-etal-2017-interactive, rocktaschel2016, jo-myaeng-2020-roles}.

\chiara{do I need a transition here, or a statement/outline of what we will do?}\\
\ev{I would have a short transition sentence here or right under the next header}

%Self-attention weights have been widely used to track token-to-token interactions, revealing that specific attention heads may be linked to distinct linguistic functions (e.g., \citealp{clark-etal-2019-bert, kovaleva-etal-2019-revealing, reif2019, lin-etal-2019-open, attention2017, voita-etal-2019-analyzing, xu2015, wang2016, lee-etal-2017-interactive, rocktaschel2016, jo-myaeng-2020-roles}). 
%Nonetheless, the reliability of raw attention weights has been recently debated \citep{jain-wallace-2019-attention, bibal-etal-2022-attention}. Attention often prioritizes uninformative tokens \citep{voita-etal-2018-context, clark-etal-2019-bert}, such as punctuation, stopwords or special tokens, making it difficult to derive meaningful insights. Moreover, it fails to account for other crucial components of the encoder layers (i.e., feed-forward networks, residual connections, and normalization layers), which contribute to how information is processed. To address these shortcomings, recent work has explored alternative approaches integrating additional components in the analysis \citep{kobayashi-etal-2020-attention, kobayashi-etal-2021-incorporating, modarressi-etal-2022-globenc, ferrando-etal-2022-measuring, mohebbi-etal-2023-quantifying}. Among these, \citet{mohebbi-etal-2023-quantifying} introduced Value Zeroing, a particularly promising method, which estimates context mixing by selectively zeroing out the value vector of a token and computing the cosine distance between the original and alternative representation of the target word. Unlike traditional attention-based methods, this technique integrates outputs from all components within Transformer layers - including residual connections and feed-forward networks - to yield more reliable context mixing measures, while preserving the original attention distribution. 

%Building on these insights, our study leverages interpretability techniques to analyze gender encoding in MT models, focusing on how gender cues (e.g., pronouns in the source sentence) influence the representation of ambiguous profession nouns. We introduce Minimal Pair Accuracy (MPA) as an evaluation metric to assess whether models consistently leverage contextual gender cues for disambiguation, moving beyond traditional gender accuracy metrics. Furthermore, we conduct an an exploratory analysis of context mixing by combining self-attention weights and value zeroing scores, examining whether specific layers or attention heads disproportionately contribute to gender encoding.
